String Stable Integral Control of Vehicle Platoons with Actuator Dynamics and Disturbances

This paper presents the design of an integral controller for vehicle platoons with actuator dynamics. The proposed controller ensures string stability with disturbances and simultaneously compensates for constant disturbances through integral action. Sufficient conditions for string stability are satisfied by the use of a suitable state transformation. The proposed controller guarantees disturbance string stability for a prescribed time constant of the actuator dynamics, and we show through simulation that platoons with faster dynamics are also made disturbance string stable.

==> figs/200330_1930normstime_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{00000}[cl][cl]{\matlabtextA C1}%
\psfrag{00001}[cl][cl]{\matlabtextA C2}%
\psfrag{0000000000002}[cl][cl]{\matlabtextA Bound (17)}%
\psfrag{0000000000003}[cl][cl]{\matlabtextA Bound (12)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{014}[bc][bc]{\matlabtextB $\sup_i\left|x_i-x_i^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $30$}%
\psfrag{008}[ct][ct]{\matlabtextC $40$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $50$}%
\psfrag{012}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> figs/200330_2018normstime_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{00000}[cl][cl]{\matlabtextA C1}%
\psfrag{00001}[cl][cl]{\matlabtextA C2}%
\psfrag{0000000000002}[cl][cl]{\matlabtextA Bound (17)}%
\psfrag{0000000000003}[cl][cl]{\matlabtextA Bound (12)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{014}[bc][bc]{\matlabtextB $\sup_i\left|x_i-x_i^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $30$}%
\psfrag{008}[ct][ct]{\matlabtextC $40$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $50$}%
\psfrag{012}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> figs/200330_2021normstime_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8.55}{8.55}\selectfont\strut}%
\psfrag{00000}[cl][cl]{\matlabtextA C1}%
\psfrag{00001}[cl][cl]{\matlabtextA C2}%
\psfrag{0000000000002}[cl][cl]{\matlabtextA Bound (17)}%
\psfrag{0000000000003}[cl][cl]{\matlabtextA Bound (12)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextB Time [s]}%
\psfrag{014}[bc][bc]{\matlabtextB $\sup_i\left|x_i-x_i^*\right|_2$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $10$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $30$}%
\psfrag{008}[ct][ct]{\matlabtextC $40$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $50$}%
\psfrag{012}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> figs/200330_2049normsN_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10.45}{10.45}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextA N}%
\psfrag{017}[bc][bc]{\matlabtextA $\sup_i\left|x_i-x_i^*\right|_\infty$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9.50}{9.50}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $50$}%
\psfrag{001}[ct][ct]{\matlabtextB $100$}%
\psfrag{002}[ct][ct]{\matlabtextB $150$}%
\psfrag{003}[ct][ct]{\matlabtextB $200$}%
\psfrag{004}[ct][ct]{\matlabtextB $250$}%
\psfrag{005}[ct][ct]{\matlabtextB $300$}%
\psfrag{006}[ct][ct]{\matlabtextB $350$}%
\psfrag{007}[ct][ct]{\matlabtextB $400$}%
\psfrag{008}[ct][ct]{\matlabtextB $450$}%
\psfrag{009}[ct][ct]{\matlabtextB $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB $2$}%
\psfrag{012}[rc][rc]{\matlabtextB $4$}%
\psfrag{013}[rc][rc]{\matlabtextB $6$}%
\psfrag{014}[rc][rc]{\matlabtextB $8$}%
\psfrag{015}[rc][rc]{\matlabtextB $10$}%
%
%% </ytick>

==> figs/200330_2210displacements10_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{7.20}{7.20}\selectfont\strut}%
\psfrag{00000}[cl][cl]{\matlabtextA C1}%
\psfrag{00001}[cl][cl]{\matlabtextA C2}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{011}[tc][tc]{\matlabtextB Time [$s$]}%
\psfrag{012}[bc][bc]{\matlabtextB $e_{1,0}$ [m]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $10$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $40$}%
\psfrag{007}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $-10$}%
\psfrag{009}[rc][rc]{\matlabtextC $-5$}%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
%
%% </ytick>

==> figs/200330_2210displacementsii-1_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{020}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{021}[bc][bc]{\matlabtextA $e_{i,i-1}$ [m]}%
\psfrag{022}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{023}[bc][bc]{\matlabtextA $e_{i,i-1}$ [m]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{010}[ct][ct]{\matlabtextB $0$}%
\psfrag{011}[ct][ct]{\matlabtextB $5$}%
\psfrag{012}[ct][ct]{\matlabtextB $10$}%
\psfrag{013}[ct][ct]{\matlabtextB $15$}%
\psfrag{014}[ct][ct]{\matlabtextB $20$}%
\psfrag{015}[ct][ct]{\matlabtextB $25$}%
\psfrag{016}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $-2$}%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $2$}%
\psfrag{009}[rc][rc]{\matlabtextB $4$}%
\psfrag{017}[rc][rc]{\matlabtextB $-20$}%
\psfrag{018}[rc][rc]{\matlabtextB $0$}%
\psfrag{019}[rc][rc]{\matlabtextB $20$}%
%
%% </ytick>

==> figs/200330_2210integralstate_control_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{018}[tc][tc]{\matlabtextA Time [s]}%
\psfrag{019}[bc][bc]{\matlabtextA $\bar{u}_i$}%
\psfrag{020}[tc][tc]{\matlabtextA Time [s]}%
\psfrag{021}[bc][bc]{\matlabtextA $\zeta_i$}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{009}[ct][ct]{\matlabtextB $0$}%
\psfrag{010}[ct][ct]{\matlabtextB $10$}%
\psfrag{011}[ct][ct]{\matlabtextB $20$}%
\psfrag{012}[ct][ct]{\matlabtextB $30$}%
\psfrag{013}[ct][ct]{\matlabtextB $40$}%
\psfrag{014}[ct][ct]{\matlabtextB $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $-4$}%
\psfrag{007}[rc][rc]{\matlabtextB $-2$}%
\psfrag{008}[rc][rc]{\matlabtextB $0$}%
\psfrag{015}[rc][rc]{\matlabtextB $-10$}%
\psfrag{016}[rc][rc]{\matlabtextB $-5$}%
\psfrag{017}[rc][rc]{\matlabtextB $0$}%
%
%% </ytick>

==> figs/200330_2210vel_accel_500.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8.80}{8.80}\selectfont\strut}%
\psfrag{019}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{020}[bc][bc]{\matlabtextA $f_i$ [kg m/s$^2$]}%
\psfrag{021}[tc][tc]{\matlabtextA Time [$s$]}%
\psfrag{022}[bc][bc]{\matlabtextA $\dot{q}_i$ [m/s]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8.00}{8.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{010}[ct][ct]{\matlabtextB $0$}%
\psfrag{011}[ct][ct]{\matlabtextB $10$}%
\psfrag{012}[ct][ct]{\matlabtextB $20$}%
\psfrag{013}[ct][ct]{\matlabtextB $30$}%
\psfrag{014}[ct][ct]{\matlabtextB $40$}%
\psfrag{015}[ct][ct]{\matlabtextB $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $16$}%
\psfrag{007}[rc][rc]{\matlabtextB $18$}%
\psfrag{008}[rc][rc]{\matlabtextB $20$}%
\psfrag{009}[rc][rc]{\matlabtextB $22$}%
\psfrag{016}[rc][rc]{\matlabtextB $-4$}%
\psfrag{017}[rc][rc]{\matlabtextB $-2$}%
\psfrag{018}[rc][rc]{\matlabtextB $0$}%
%
%% </ytick>
